SNIP: Bridging Mathematical Symbolic and Numeric Realms with Unified Pre-training

In an era where symbolic mathematical equations are indispensable for modeling complex natural phenomena, scientific inquiry often involves collecting observations and translating them into mathematical expressions. Recently, deep learning has emerged as a powerful tool for extracting insights from data. However, existing models typically specialize in either numeric or symbolic domains, and are usually trained in a supervised manner tailored to specific tasks. This approach neglects the substantial benefits that could arise from a task-agnostic multi-modal understanding between symbolic equations and their numeric counterparts. To bridge the gap, we introduce SNIP, a Symbolic-Numeric Integrated Pre-training model, which employs contrastive learning between symbolic and numeric domains, enhancing their mutual similarities in the embeddings. By performing latent space analysis, we observe that SNIP provides cross-domain insights into the representations, revealing that symbolic supervision enhances the embeddings of numeric data and vice versa. We evaluate SNIP across diverse tasks, including symbolic-to-numeric mathematical property prediction and numeric-to-symbolic equation discovery, commonly known as symbolic regression. Results show that SNIP effectively transfers to various tasks, consistently outperforming fully supervised baselines and competing strongly with established task-specific methods, especially in the low data regime scenarios where available data is limited. Code and model are available at: https://github.com/deep-symbolic-mathematics/Multimodal-Math-Pretraining

==> Arxiv/fig_table_tex/fig_bbox_pairgrid.tex <==


\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\linewidth]{Arxiv/fig_table_file/snip_median_pairgrid-pointplot_r2_test_model_size.png}
% \captionsetup{font=footnotesize}
\caption{Performance comparison of \modelname and SRBench algorithms on the \textit{Black-box} dataset in terms of Accuracy-Complexity-Time. Models are ranked by mean accuracy, quantified as the proportion of test solutions with $R^2>0.99$ across varying target noise levels. Error bars denote the $95\%$ confidence interval.
\vspace{-1.0em}
}
\vspace{-0.5em}
\label{fig:srbboxpg}
\end{figure}

==> Arxiv/fig_table_tex/fig_extrap_qualres.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{Arxiv/fig_table_file/extrap_examples_v1.jpg}
% \captionsetup{font=footnotesize}
\caption{Qualitative results of extrapolation on function examples for Transformers encoder-decoder models ($i$) without pre-training; ($ii$) with frozen \modelname's numeric encoder; and with ($iii$) fine-tuned \modelname's numeric encoder, highlighted with \textcolor{red}{red}, \textcolor{blue}{blue}, and \textcolor{darkergreen}{green} lines, respectively.
% \vspace{-1.0em}
}
\label{fig:extrapqual}
\end{figure}

==> Arxiv/fig_table_tex/fig_fewshot.tex <==



\begin{wrapfigure}[16]{r}{0.3\linewidth}
% \begin{figure}[t]
\centering
\vspace{-3.4em}
\includegraphics[width=\linewidth]{Arxiv/fig_table_file/fewshot.png}
% \captionsetup{font=footnotesize}
\caption{\small $R^2$ scores for \textit{NCR} property prediction task vs. the number of training samples. 
% Both frozen and finetuned 
\modelname variants outperform the supervised model, with the performance gap widening in few-shot scenarios with limited training data.
% Testing $R^2$ of \textit{NCR} property prediction task vs. number of samples in the dataset. \modelname (without and with finetuning) outperforms the supervised model with a higher margin on smaller training datasets (\textbf{few-shot scenarios}).
\vspace{-1.5em}
}
\label{fig:fewshot}
\vspace{-0.8em}
% \end{figure}
\end{wrapfigure}

==> Arxiv/fig_table_tex/fig_feyn_pairgrid.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\linewidth]{Arxiv/fig_table_file/snip_feyn_pairgrid20_wnoise_accuracy_r2_0.99_model_size_training-time-(s).png}
% \captionsetup{font=footnotesize}
\caption{Performance comparison of \modelname and SRBench algorithms on the \textit{Feynman} dataset in terms of Accuracy-Complexity-Time. Models are ranked by mean accuracy, quantified as the proportion of test solutions with $R^2>0.99$ across varying target noise levels. Error bars denote the $95\%$ confidence interval.
\vspace{-1.0em}
}
\vspace{-0.5em}
\label{fig:srfeynpg}
\end{figure}

==> Arxiv/fig_table_tex/fig_latent_properties_1d.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.98\linewidth]{Arxiv/fig_table_file/latent_properties2.pdf}
% \captionsetup{font=footnotesize}
\caption{\small 2D t-SNE plots of the latent space of pretrained SNIP on 1D datasets. \textbf{(a-d)} Symbolic Encoded vectors $Z_f$ colored by numeric properties: (a) Non-Convexity Ratio (NCR), (b) Oscillations, (c) Average of Normalized $y$, and (d) Upwardness. \textbf{(e-f)} Numeric encoded vectors $Z_y$ colored by symbolic properties: (e) Function Complexity, and (f) Function Classes based on Operators.
\vspace{-1.0em}
}
\label{fig:latentprop_1d_appendix}
\end{figure}

==> Arxiv/fig_table_tex/fig_latent_property.tex <==



\begin{wrapfigure}[19]{r}{0.55\linewidth}
% \begin{figure}[t]
\centering
\vspace{-1.5em}
\includegraphics[width=\linewidth]{Arxiv/fig_table_file/latent_finetune3.pdf}
% \captionsetup{font=footnotesize}
\caption{\small 2D t-SNE plots of the encoded representations for \textbf{(top)} Non-Convexity Ratio and \textbf{(bottom)} Function Upwardness prediction tasks, comparing  \textbf{(a)} supervised models without pretraining, \textbf{(b)} frozen pretrained \modelname encoder, and \textbf{(c)} fine-tuned \modelname encoders for each task.
% 2D t-SNE plots of the encoded vectors for the tasks of \textbf{(top)} Non-Convexity Ratio (NCR) and \textbf{(bottom)} Function Upwardness prediction. The latent representations are shown for \textbf{(a)} fully supervised model without pretrained \modelname, \textbf{(b)} pretrained \modelname encoder, and \textbf{(c)} the pretrained \modelname encoder after fine-tuning for the specific property prediction task.
\vspace{-1.5em}
}
\label{fig:latentprop}
\vspace{-0.7em}
% \end{figure}
\end{wrapfigure}

==> Arxiv/fig_table_tex/fig_sr_indomain_comp.tex <==


% \begin{figure}[t]
% \centering
% % \vspace{-1.5em}
% \includegraphics[width=\linewidth]{Arxiv/fig_table_file/comp_detailed_indomain.jpg}
% \vspace{-1.0em}
% \caption{\textcolor{blue}{\small Detailed Performance Evaluation of \textbf{Mean Expression Complexity} between \modelname and E2E Transformer baseline across 400 Synthetic Validation Functions for different levels of formula and input difficulties: \textbf{(a) number of binary operators, (b) number of unary operators, (c) input dimension, and (d) number of input centroids.} 
% % Performance comparison of \modelname and E2E transformer baseline in terms of mean accuracy defined as the ratio of solutions with $R^2>0.99$ over $400$ in-domain synthetic validation functions
% % across different levels of formula and input difficulties: \textbf{(a) number of binary operators, (b) number of unary operators, (c) input dimension, and (d) number of input centroids.}
% }}
% \label{fig:sr-indomain-comp}
% \vspace{-0.5em}
% \end{figure}

==> Arxiv/fig_table_tex/fig_stro_pairgrid.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\linewidth]{Arxiv/fig_table_file/snip_stro_pairgrid9_wnoise_accuracy_r2_0.99_model_size_training-time-(s).png}
% \captionsetup{font=footnotesize}
\caption{Performance comparison of \modelname and SRBench algorithms on the \textit{Strogatz} dataset in terms of Accuracy-Complexity-Time. Models are ranked by mean accuracy, quantified as the proportion of test solutions with $R^2>0.99$ across varying target noise levels. Error bars denote the $95\%$ confidence interval.
% Performance comparison of \modelname and SRBench algorithms in terms of Accuracy-Complexity-Time on \textit{Strogatz} dataset. Models are sorted based on mean accuracy defined as the ratio of solutions with $R^2>0.99$ on test set under various noise levels $\gamma \in \{0, 0.001, 0.01, 0.1\}$. The error bars represent the $95\%$ confidence interval.
% Performance comparison of \modelname and SRBench algorithms in terms of Accuracy-Complexity-Time on \textit{Strogatz} datasets.
\vspace{-1.0em}
}
\vspace{-0.5em}
\label{fig:srstropg}
\end{figure}

==> Arxiv/fig_table_tex/table_extrap.tex <==
% \vspace{-0.5em}
\begin{table}[ht]
\begin{center}
 \aboverulesep=0ex
 \belowrulesep=0ex
 % \renewcommand{\arraystretch}{1.0}
% \setlength{\tabcolsep}{7.0pt}
\renewcommand{\arraystretch}{0.9}
% \scriptsize
% \rmfamily
\centering
% \hskip-0.3cm
\small
\caption{\label{tab:extrapquant} Results of extrapolation task}
% \vspace{-1.5em} }
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
Model & $\downarrow$\textit{MAE} & $\downarrow$\textit{RMSE} & $\downarrow$\textit{MAPE}(\%) \\
\midrule
Supervised&  0.154&  0.192& 28.935 \\
% \midrule
\modelname (frozen) &  0.117&  0.135& 16.304  \\
\modelname (finetuned) &  \textbf{0.096}&  \textbf{0.118}& \textbf{13.349} 
\\
\hline
\arrayrulecolor{black}\bottomrule
\end{tabular}
}
\end{center}
% \vspace{-0.5em}
\end{table}

==> Arxiv/sections/discussion.tex <==
\vspace{-0.5em}
\section{Discussion}
\vspace{-0.5em}
\label{sec:discussion}

==> Arxiv/sections/experiments.tex <==
\vspace{-0.5em}
\section{Experiments}
\label{sec:experiments}

% \subsection{Function Integration (S2S)}
% \subsubsection{Task Definition}
% \subsubsection{Task Formulation and Data Construction}
% \subsubsection{Model Comparisons}

% \subsection{Numeric-to-Numeric}

% \subsection{Interpolation}
% \subsubsection{Task Definition and Formulation}
% \subsubsection{Data Construction}
% \subsubsection{Model Comparisons}

% \subsection{Extrapolation}
% \subsubsection{Task Definition and Formulation}
% We aim to validate the quality of \modelname's numeric encoded representations with the out-of-distribution extrapolation downstream task. This task essentially involves the numeric forecasting of values for a mathematical function outside the given range of observed values, a task that we model as a sequence-to-sequence problem. Given a set of numeric inputs $(x_W,y_W)\in\mathbb{R}^{D+1}$ where $x_W \in \mathcal{D}_{W}$ and $y_W=f(x_W)$, our objective is to predict the future values of the function for the new subsequent range, based on these historical observed values. In this scenario, $\mathcal{D}_{W}$ refers to the observed range of independent variables. In terms of the task formulation, the target is to compute $\hat{y}_{H}=\mathcal{F}(x_W,y_W)$, where $\hat{y}_H$ are the predicted future values of the target variable and $\mathcal{F}(x_W,y_W)$ refers to the seq2seq model composed of the \modelname's numeric encoder and a numeric decoder $Dec^V$, specifically designed for this task. In other words, we have $\hat{y}_H = Dec^{V}(\bm{Z}^V)$ where $\bm{Z}^V = \text{AttentionPool}\left(Enc^V(x_W,y_W)\right)$ represents the encoded sequence-level representations of given values $(x_W,y_W)$, obtained from the \modelname's pre-trained numeric encoder $Enc^V$. The ideal future range values are derived from the underlying function of the samples provided with independent variables in the new range, i.e., $y_H = f(x_H)$ for $x_H\in\mathcal{D}_{H}$, such that $\mathcal{D}_{H}\cap\mathcal{D}_W=\emptyset$ meaning that the historical observed sample range does not intersect with the future prediction range, thereby emphasizing the extrapolation/forecasting aspect of task. Training of this model is conducted via minimizing the Mean-Squared-Error (MSE) loss function $\mathcal{L}_{MSE} = \frac{1}{M} \sum_{j=1}^{M} (\hat{y}^j_{H}-y^j_{H})^2$ with $M$ denoting the prediction horizon (i.e., number of points in the new range); and $j$ being an individual prediction point. While the decoder $Dec^V$ is specifically trained for this task, the \modelname's pre-trained numeric encoder $Enc^V$ can either be kept frozen or fine-tuned during this training process. Both configurations will be investigated in our experiments. 
% It's crucial to note that the underlying function $f(\cdot)$ of the samples is known only during the training process to calculate the ground-truth target values $y_H$ and compute the loss. However, during inference, this function is unknown, and only the input data pairs $(x_W,y_W)$ are fed to the model to predict out-of-distribution target values $\hat{y}_{H}$. 
% The structure and training strategy of this task, drawing points from various $f$, is devised as a zero-shot seq2seq forecasting model that can predict values for samples from any function $f$ at inference, without requiring additional training or fine-tuning for new functions.
% % It's important to note that the structure and training of this task (with samples from various $f$) is designed as a zero-shot capable seq2seq forecasting model that can make predictions for samples coming from any function $f$ at inference without the need of training/fine-tuning for a data from a new function. 
% This downstream task underscores the wide-ranging applicability potential of \modelname in scenarios involving numeric prediction, leveraging its rich semantic features, which have been trained with the corresponding mathematical function context. This imparts \modelname with superior capabilities for extrapolation outside of distribution, correlating tightly with the true symbolic and mathematical patterns hidden in the data, which may not be necessarily visible from the observed values. 
% % , capitalizing on its rich semantic features trained with a mathematical function context, making it best for out-of-distribution extrapolation capabilities, which correlate closely with the true symbolic and mathematical patterns in the data which are not necessarily visible from the existing observed values.

% % due to containing rich semantic features which were trained with mathematical function context, making it best for out-of-distribution extrapolation capability which is closely related to the true symbolic and mathematical patterns in the data.
% % understanding the true symbolic and mathematical patterns in the data, which helps the model to have better out-of-distribution extrapolation capability.   


% % tly proposed CLIP model contains rich semantic features which were trained with textual context, making it
% % best for vision-language perception


% % the zero-shot learning capability of the trained $\mathcal{F}$ model for samples coming from any function $f$ during inference. 


% % our model \modelname and underscores the model's potential for broader application in numeric forecasting scenarios.



% % We validate the quality of \modelname's numeric encoded representations with the out-of-distribution extrapolation downstream task which is the task of numeric forecasting for values of a mathematical function outside the given range for observed values. This task can be conceptualized as a sequence-to-sequence (seq2seq) problem that involves numeric inputs of $(x_W,y_W)\in\mathbb{R}^{D+1}$ for $x_W \in \mathcal{D}_{W}$ where $y_W=f(x_W)$ and $\mathcal{D}_{W}$ refers to the given range of observed values for independent variables. In this task, the goal is to predict the future values of this function (which are within a new range) based on historical observed values, i.e., $\hat{y}_{H}=\mathcal{F}(x_W,y_W)$ where $\hat{y}_H$ refers to the predicted future values of the target variable; and $\mathcal{F}(x_W,y_W)$ is the seq2seq model containing the \modelname's numeric encoder and the numeric decoder $Dec^V$ that has been designed for this task. So, we have $\hat{y}_H = Dec^{V}(\bm{Z}^V)$ with $\bm{Z}^V = \text{AttentionPool}\left(Enc^V(x_W,y_W)\right)$ referring to the encoded sequence-level representations of given values $(x_W,y_W)$ obtained from the \modelname's pre-trained numeric encoder $Enc^V$. The ideal values for the future range are the target values obtained from the underlying function of the samples given the independent variables in the new range, i.e., $y_H = f(x_H)$ for $x_H\in\mathcal{D}_{H}$ where $D_{H}\cap\mathcal{D}_W=\emptyset$ meaning that the range of independent variables in the historical observed samples doesn't intersect with their prediction range (i.e., task of extrapolation/forecasting). We train this model with the Mean-Squared-Error (MSE) loss function, so, $\mathcal{L} = \min_{\theta}(\hat{y}_{H}-y_{H})^2$ in which we can only train the decoder designed for this task and keep the \modelname's pre-trained encoder frozen, or we can also fine-tune encoder in the training process. It's important to note that the underlying function of samples $f(\cdot)$ is only known during training to calculate the ground-truth target values $y_H$ and find the loss. However, this function is unknown during inference, and we only feed input sample pairs $(x_W,y_W)$ to predict out-of-distribution target values $\hat{y}_{H}$. 

% \subsubsection{Data Construction}
% For this task, we first sample a function $f$ following the strategy used in Section~\ref{sec:pretrain_data} for function sampling. This allows us to generate a diverse dataset representative of various mathematical functions. Then for each function $f$, $N$ numeric input points are sampled with the same step size $\delta_W$ in the given input range $[{min}_W,{max}_W]$, i.e., $x^0_W={min}_W$, and $\left(x^i_W = x^{i-1}_W+\delta_W\right)^N_{i=1}$ for  $\delta_W=\lfloor{({max}_W - {min}_W)/N}\rfloor$.
% % i.e., $x^i_W \in [{min}_W,{max}_W]^{D}$ for $i=1,\ldots,N$.
% % Then, we can find the target value for each point: $y^i_W=f(x^i_W)$.
% In this task, input of the encoder consists of an $(x_W,y_W)\in\mathbb{R}^{D+1}$ pair, where $y^i_W=f(x^i_W)$ for each input point. After finding \modelname's numeric encoded representations for input $(x_W,y_W)$, we use a decoder on top of it to predict $M$ target values in the output range $[{min}_H,{max}_H]$. In other words, for training decoder to effectively predict target values with step size $\delta_H$ in the new unseen range, we use the actual future values of function $\left(y^j_H=f(x^j_H)\right)^M_{j=1}$, where $x^0_H = {min}_H$ and $x^j_H = x^{j-1}_H+\delta_H$ for $\delta_H=\lfloor (max_H - min_H)/M \rfloor$. 
% % $x^j_H\in[{min}_H,{max}_H]^D$. 
% In our experiments, we set the input range $[{min}_W,{max}_W]=[1,4)$ and the output range $[{min}_H,{max}_H]=[4,4.75)$. We also set the number of input points for each function $N=200$, and the number of prediction points as $M=50$, leading to the same step size $\delta_W=\delta_H=0.015$ for both inputs and outputs. We also use $100$k sampled functions for training and $10$k different sampled functions for evaluation. 

% % For training deocder to effectively predict target values outside the given input range, we use $y_H=f(x_H)$ where $x_H\in[{min}_H,{max}_H]$

% % $x^i_W:i=1,\ldots,N$ are sampled from $f$, where $x_W\in [{min}_W,{max}_W]^{D}$. These $N$ points are sampled with the same distance in the given input range. In our experiments, we take ${min}_W=1$ and ${max}_W=4$. Then, we can find the target value $y^i_W=f(x^i_W)$. 

% \subsubsection{Model Comparisons}
% In order to highlight the efficacy of \modelname's pre-trained numeric encoder, we experiment with three variants of the encoder-decoder model: $(i)$ a vanilla model without any pre-training (being trained on this task from scratch with randomly initialized parameters); $(ii)$ a model where the numeric encoder remains frozen to the \modelname's pre-trained weights during fine-tuning process (only training the decoder for this downstream task); and $(iii)$ a model where the numeric encoder is initialized from \modelname's pre-trained weights and then fine-tuned alongside the decoder for this task. It's important to also note that the encoder and decoder of this model both have Transformers architecture. 
% These three models are compared based on their predictive accuracy over the output range. The metrics of evaluation include Mean Absolute Error (MAE), Root Mean Squared Error (RMSE), and Mean Absolute Percentage Error (MAPE) between the actual target values in the output range and the predicted target values generated by each model. Our key objective here is to just demonstrate that \modelname's pre-trained model and its associated encoded representations can effectively contribute to a function-agnostic out-of-range predictor, which has undergone training with a variety of $f$ samples.
% % thereby validating the efficacy of the pre-training contrastive objective. 
% % This serves as a testament to the efficiency of the pre-training contrastive objective. 
% The detailed quantitative and qualitative results of this study are provided below.   
% % out-of-range value estimator, thereby validating the efficacy of the pre-training contrastive objective. The quantitative and qualitative results of this study are provided below.  
% % The quantitative and qualitative results of this task are summarized below. 

% \noindent \textbf{Quantitative Results}
% provided below, will pave the way for further research into multi-modal pre-training models in the realm of symbolic and numeric mathematical tasks.

% \input{Arxiv/fig_table_tex/table_extrap}


% \noindent \textbf{Qualitative Results}

% \input{Arxiv/fig_table_tex/fig_extrap_qualres}

% \subsection{Symbolic Regression}
% \subsubsection{Task Definition}

% Symbolic Regression (SR) is a task that revolves around discovering a symbolic expression to represent an unknown function $f(\cdot)$. Given a $d$-dimensional input $\bm x \in \mathbb{R}^{d}$, the function maps it to the target variable $y = f(\bm x) \in \mathbb{R}$. The objective of SR is to find an equation $\hat{f}(\cdot)$ that approximates the target variable based on a dataset of $n$ observations $\mathcal{D} = (\bm x_i, y_i)_{i=1}^{n}$.

% Previous methods for SR, particularly those employing transformer-based approaches, have tackled this task in an end-to-end manner. These models are trained on a comprehensive dataset of equation instances and, during inference, generate symbolic expressions as sequences of tokens in an autoregressive manner. Techniques like beam search and sampling are used for decoding, enabling the models to generate multiple candidate equations based on the input observations. While these approaches have shown promise, challenges persist in generating accurate constants within the equations and optimizing for sequence-level objectives, such as fitting or equation complexity.

% \subsubsection{Task Formulation and Data Construction}
% \subsubsection{Model Comparisons}

\subsection{Function Property Prediction}
\subsubsection{Task Definition}
\subsubsection{Task Formulation and Data Construction}
\subsubsection{Model Comparisons}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

